Page Curves and Bath Deformations

We study the black hole information problem within a semiclassically gravitating AdS$_d$ black hole coupled to and in equilibrium with a $d$-dimensional thermal conformal bath. We deform the bath state by a relevant scalar deformation, triggering a holographic RG flow whose "trans-IR" region deforms from a Schwarzschild geometry to a Kasner universe. The setup manifests two independent scales which control both the extent of coarse-graining and the entanglement dynamics when counting Hawking degrees of freedom in the bath. In tuning either, we find nontrivial changes to the Page time and Page curve. We consequently view the Page curve as a probe of the holographic RG flow, with a higher Page time manifesting as a result of increased coarse-graining of the bath degrees of freedom.

==> Page curves bath def/figs/candidateSurfaces.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=1.1]
\draw[->] (0,2) to (2+2,2);
\draw[-,very thick,red] (0,2) to (0,0);

\draw[->] (0,2.3) to (0.5,2.3);
\node at (0,2.5) {$x^1$};

\draw[->] (-0.3,2) to (-0.3,1.5);
\node at (-0.5,1.5) {$r$};

\node at (0,-0.2) {\textcolor{red}{$x^1 = 0$}};

\draw[-,dashed] (0,0.2) to (2+2,0.2);

\node at (2+2.6,0.2) {$r = r_+$};
\node at (2+2.6,2) {$r = 0$};

\draw[-,yellow!20!orange,very thick] (1.5,2) to (1.5,0.2);
\draw[-,blue!30!teal,very thick] (1.5,2) to[bend left] (0,1.225);
\draw[-,blue!30!teal] (0.1,1.225) to (0.1,1.325) to (0,1.325);

\draw[->,very thick,black!25!lime] (1.5,2) to (4,2);
\node at (2.625,2.25) {\textcolor{black!25!lime}{$\mathcal{R}^{L,R}$}};

\draw[-,black!25!lime,thick] (1.6,2.2) to (1.5,2.2) to (1.5,1.8) to (1.6,1.8);
\node at (1.5,2.4) {\textcolor{black!25!lime}{$x_\mathcal{R}$}};

\node[color=red] at (0,2) {$\bullet$};
\node at (0,2) {$\circ$};
\end{tikzpicture}
\caption{The candidate RT surfaces in one of the exterior regions. The orange line entering the horizon is the Hartman-Maldacena surface, whereas the blue arc which ends perpendicularly on the brane is the island-producing exterior surface.}
\label{figs:candidateSurfaces}
\end{figure}

==> Page curves bath def/figs/eternalBH.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=1.65]
\node at (1.35,0.25) {\textcolor{black!25!lime}{\footnotesize$\bullet$}};
\draw[-,black!25!lime,very thick] (1.35,0.25)  .. controls (1.6,0.2) and (1.8,0.2) ..  (2.25,0);
\draw[-,draw=none,fill=white] (1,1) to (2.25,0) to (2.5,0) to (1.25,1) to (1,1);


\node at (-1.35,0.25) {\textcolor{black!25!lime}{\footnotesize$\bullet$}};
\draw[-,black!25!lime,very thick] (-1.35,0.25) .. controls (-1.6,0.2) and (-1.8,0.2) .. (-2.25,0);
\draw[-,draw=none,fill=white] (-1,1) to (-2.25,0) to (-2.5,0) to (-1.25,1) to (-1,1);


\node at (3.375/2,-0.05) {\textcolor{black!25!lime}{$\mathcal{R}^R(t_0)$}};
\node at (-3.375/2,-0.05) {\textcolor{black!25!lime}{$\mathcal{R}^L(t_0)$}};



\draw[-,draw=none,fill=black!10] (1,1) to (1,-1) to (0,0) to (1,1); 
\draw[-,draw=none,fill=black!10] (-1,1) to (-1,-1) to (0,0) to (-1,1);

\draw[-,draw=none,fill=violet!10] (-1,1) to[bend right] (1,1) to (0,0) to (-1,1); 
\draw[-,draw=none,fill=violet!10] (1,-1) to[bend right] (-1,-1) to (0,0) to (1,-1);

\draw[-,decoration = {zigzag,segment length = 1mm, amplitude = 0.25mm},decorate] (-1,1) to[bend right] (1,1);
\draw[-] (1,1) to (1,-1);
\draw[-,decoration = {zigzag,segment length = 1mm, amplitude = 0.25mm},decorate] (1,-1) to[bend right] (-1,-1);
\draw[-] (-1,-1) to (-1,1);

\draw[-,dashed] (-1,1) to (1,-1);
\draw[-,dashed] (1,1) to (-1,-1);

\draw[-] (1,-1) to (2.25,0) to (1,1) to (1,-1);
\draw[-] (-1,-1) to (-2.25,0) to (-1,1) to (-1,-1);


\draw[-,very thick,blue!30!teal] (-0.5,0.25) to (-0.25,0.25) .. controls (0,0.175) .. (0.25,0.25) to (0.5,0.25);
\node[blue!30!teal] at (-0.5,0.25) {$\bullet$};
\node[blue!30!teal] at (0.5,0.25) {$\bullet$};

\node[blue!30!teal] at (0,0.325) {$\mathcal{I}$};
\node at (0,-1.2) {};
\end{tikzpicture}
\begin{tikzpicture}[scale=0.75]
\draw[->,thick] (0,-0.2) to (0,4);
\draw[->,thick] (-0.2,0) to (6,0);

\node at (-0.6,4) {$S^{\text{ren}}$};
\node at (6.2,0) {$t$};

\draw[-,blue!30!teal,very thick] (3,2.5) to (6,2.5);
\draw[-,dashed,blue!30!teal] (0,2.5) to (3,2.5);

\draw[-,dashed,yellow!20!orange] (3,2.5) to (4.8,4);
\draw[-,yellow!20!orange,very thick] (0,0) to (3,2.5);
\node at (3,2.5) {$\circ$};
\draw[-,dashed] (3,2.5) to (3,0);
\draw[-] (3,0) to (3,-0.05);
\node at (3,-0.4) {$t_p$};


\node[yellow!20!orange] at (1,1.7) {$S_\varnothing(t_0)$};
\node[blue!30!teal] at (4.5,2.8) {$S_{\mathcal{I}}$};

\node at (-0.4,0) {$0$};
\end{tikzpicture}
\caption{On the left is the two-sided thermal configuration of (II) featuring both the $t = t_0$ radiation region $\mathcal{R}^L(t_0) \cup \mathcal{R}^R(t_0)$ and the island $\mathcal{I}$ which emerges at late times. The right figure is a sketch of the (eternal) Page curve depicting (renormalized) entanglement entropy versus time---initially the time-dependent no-island entropy $S_\varnothing$ is minimal, but it eventually exceeds the non-trivial island entropy $S_{\mathcal{I}}$. This curve can be obtained by computing (renormalized) areas in the (III) configuration.}
\label{figs:eternalBH}
\end{figure}

==> Page curves bath def/figs/islands.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=1]
\draw[->] (0,2) to (2+2,2);
\draw[-,red] (0,2) to (-1,0);

\draw[->,very thick,black!25!lime] (1.5,2) to (4,2);
\node[black!25!lime] at (1.5,2) {$\bullet$};
\node at (2.75,2.2) {\textcolor{black!25!lime}{$\mathcal{R}$}};


\draw[-,very thick,black!25!lime,dashed] (1.5,2) arc (0:-117:1.5);

\draw[-,blue!30!teal,very thick] (0-0.675,2-0.675*2) to (-1,0);

\node[blue!30!teal] at (0-0.675,2-0.675*2) {$\bullet$};
\node[blue!30!teal] at (-6.5/8-0.2,0.375) {$\mathcal{I}$};

%\draw[-,black!25!lime,thick] (1.6,2.2) to (1.5,2.2) to (1.5,1.8) to (1.6,1.8);


\draw[->,decoration = {zigzag,segment length = 1mm, amplitude = 0.25mm},decorate] (0.1-0.5,1) .. controls (0+0.1,2-0.1) .. (1,1.9);
\node[rotate=180-30,scale=0.75] at (0.1-0.5,1) {$\blacktriangle$};
\node[rotate=-90,scale=0.75] at (1,1.9) {$\blacktriangle$};

\node[color=red] at (0,2) {$\bullet$};
\node[] at (0,2) {$\circ$};
\end{tikzpicture}
\caption{A cartoon depiction of the setup, with the brane in red, the bath in black, and the interface represented as a dot. The two-headed arrow indicates transparent boundary conditions. By computing the entanglement entropy of the radiation region $\mathcal{R}$, the island rule demands that we \textit{also} minimize over possible regions on the brane $\mathcal{I}$. Classically in (III), we end up with the $\mathcal{I}$ for which the entanglement surface area (possibly including brane-action contributions) is minimal.}
\label{figs:islands}
\end{figure}

==> Page curves bath def/figs/kasnerVsDef/kasnerVsDef.tex <==
\begin{figure}
\centering
\subfloat[d=2]{
\includegraphics[scale=0.5]{figs/kasnerVsDefd3.pdf}}
\quad
\subfloat[d=2]{
\includegraphics[scale=0.5]{figs/kasnerVsDefd3.pdf}}
\quad
\subfloat[d=2]{
\includegraphics[scale=0.5]{figs/kasnerVsDefd3.pdf}}
\caption{(a) The area difference $\Delta\mathcal{A}(0)$ \eqref{areaDiff} versus $x_\mathcal{R}$ \eqref{radEnd} for various dimensions $d$ and (b) the Page point $x_p$ as a function of $d$, all in the AdS-Schwarzschild geometry with $r_+ = 2$. The area difference in each dimension monotonically increases for larger and larger $x_\mathcal{R}$, crossing $0$ at a particular value beyond which we have Page curves. This confirms a $d$-dependent Page point which goes closer to the brane as we increase $d$. Fixing $r_+$ simply sets a scale.}
\label{figs:pagePointAS}
\end{figure}

==> Page curves bath def/figs/pagePointAS/pagePointAS.tex <==
\begin{figure}
\centering
\subfloat[Area difference]{
\includegraphics[scale=0.5]{figs/areaDiffAdSSchwarzschild.pdf}}
\quad
\subfloat[Page point]{
\includegraphics[scale=0.5]{figs/pagePointAdSSchwarzschild.pdf}}
\caption{(a) The area difference $\Delta\mathcal{A}(0)$ \eqref{areaDiff} versus $x_\mathcal{R}$ \eqref{radEnd} for various dimensions $d$ and (b) the Page point $x_p$ as a function of $d$, all in the AdS-Schwarzschild geometry with $r_+ = 2$. The area difference in each dimension monotonically increases for larger and larger $x_\mathcal{R}$, crossing $0$ at a particular value beyond which we have Page curves. This confirms a $d$-dependent Page point which goes closer to the brane as we increase $d$. Fixing $r_+$ simply sets a scale.}
\label{figs:pagePointAS}
\end{figure}

==> Page curves bath def/figs/volcanoPotential.tex <==
\begin{figure}
\centering
\includegraphics[scale=0.85]{figs/volcanoPot.pdf}
\caption{A sketch of the AdS volcano potential $V(w)$ in \cite{Karch:2000ct} for $d = 4$, depicted as a function of a coordinate $w$ which is normal to the brane. We show both the $T > 0$ case (which has a crater) and the $T = 0$ case (which lacks a crater).}
\label{figs:volcanoPotential}
\end{figure}

==> Page curves bath def/tables/asymptoticExpressions.tex <==
\begin{table}
\centering
\begin{tabular}{c||c|c}{}
& Near-boundary ($r \to 0$) & Near-singularity ($r \to \infty$)\\\hline\hline & & \vspace{-1em}\\
$\underset{(\Delta \neq d/2)}{\phi(r)}$ & $\phi_0 r^{d-\Delta} + \dfrac{\expval{\mathcal{O}}}{2\Delta - d} r^\Delta$ & $\sqrt{2(d-1)(\rho - d)}\log r$\\ & & \vspace{-1em}\\ \hline & &\vspace{-1em}\\
$\underset{(\Delta = d/2)}{\phi(r)}$ & $\phi_0 r^{d/2}\log r$ & $\sqrt{2(d-1)(\rho - d)}\log r$\\ & & \vspace{-1em}\\ \hline & &\vspace{-1em}\\
$\underset{(\Delta \neq d/2)}{\chi(r)}$ & $\dfrac{d-\Delta}{2(d-1)}\phi_0^2 r^{2(d-\Delta)} + \dfrac{2\Delta(d-\Delta)}{d(d-1)(2\Delta - d)}\phi_0\expval{\mathcal{O}}r^d$ & $2(\rho-d) \log r + \chi_1$\\
& $ \qquad\qquad\qquad\qquad+ \dfrac{\Delta}{2(d-1)(2\Delta-d)^2}\expval{\mathcal{O}}^2 r^{2\Delta}$ & \\ & & \vspace{-1em}\\ \hline & &\vspace{-1em}\\
$\underset{(\Delta = d/2)}{\chi(r)}$ & $\dfrac{\phi_0^2}{4d(d-1)} r^d \left[2 + 2d\log r + d^2 (\log r)^2\right]$ & $2(\rho-d) \log r + \chi_1$\\ & & \vspace{-1em}\\ \hline & &\vspace{-1em}\\
$f(r)$ & $e^{\chi(r)}\left(1 - \expval{T_{tt}}r^d\right)$ & $-f_1 r^{\rho}$
\end{tabular}
\caption{The near-boundary and near-singularity expressions for the radial functions characterizing a Kasner flow ansatz for the Einstein + scalar theory. The near-boundary data is controlled by the deformation parameter $\phi_0/T^{d-\Delta}$ while all of the near-singularity data is determined by the Kasner exponent $p_t$.}
\label{tables:asymptoticExpressions}
\end{table}

==> figs/kasnerVsDef/kasnerVsDef.tex <==
\begin{figure}
\centering
\subfloat[d=2]{
\includegraphics[scale=0.5]{figs/kasnerVsDefd3.pdf}}
\quad
\subfloat[d=2]{
\includegraphics[scale=0.5]{figs/kasnerVsDefd3.pdf}}
\quad
\subfloat[d=2]{
\includegraphics[scale=0.5]{figs/kasnerVsDefd3.pdf}}
\caption{(a) The area difference $\Delta\mathcal{A}(0)$ \eqref{areaDiff} versus $x_\mathcal{R}$ \eqref{radEnd} for various dimensions $d$ and (b) the Page point $x_p$ as a function of $d$, all in the AdS-Schwarzschild geometry with $r_+ = 2$. The area difference in each dimension monotonically increases for larger and larger $x_\mathcal{R}$, crossing $0$ at a particular value beyond which we have Page curves. This confirms a $d$-dependent Page point which goes closer to the brane as we increase $d$. Fixing $r_+$ simply sets a scale.}
\label{figs:pagePointAS}
\end{figure}

==> figs/pagePointAS/pagePointAS.tex <==
\begin{figure}
\centering
\subfloat[Area difference]{
\includegraphics[scale=0.5]{figs/areaDiffAdSSchwarzschild.pdf}}
\quad
\subfloat[Page point]{
\includegraphics[scale=0.5]{figs/pagePointAdSSchwarzschild.pdf}}
\caption{(a) The area difference $\Delta\mathcal{A}(0)$ \eqref{areaDiff} versus $x_\mathcal{R}$ \eqref{radEnd} for various dimensions $d$ and (b) the Page point $x_p$ as a function of $d$, all in the AdS-Schwarzschild geometry with $r_+ = 2$. The area difference in each dimension monotonically increases for larger and larger $x_\mathcal{R}$, crossing $0$ at a particular value beyond which we have Page curves. This confirms a $d$-dependent Page point which goes closer to the brane as we increase $d$. Fixing $r_+$ simply sets a scale.}
\label{figs:pagePointAS}
\end{figure}
